Gatling: Rapid-Fire Consensus from Parallel Composition

Consensus protocols form the core of blockchains and other replicated state machines, ensuring that all correct nodes process the same totally ordered log of input transactions. In fault-free executions, performance is driven by the good-case transaction latency -- the time between a transaction becoming known to all nodes and its confirmation by the consensus protocol -- which depends on both how frequently proposals are made and, once made, how quickly they are confirmed. While prior work has established tight lower bounds on confirmation latency that modern protocols already achieve, it remains open whether the inter-proposal time can be further reduced below the state-of-the-art of one network delay. We introduce Gatling, an atomic broadcast protocol that achieves arbitrarily small inter-proposal times under rotating leader schedules; in particular, smaller than the network delay. Gatling runs multiple parallel instances of a black-box atomic broadcast protocol and staggers their proposal schedules to generate proposals in faster succession than state-of-the-art protocols. A deterministic interleaving rule merges the outputs of these instances into a single global log. We analyze the effects of head-of-line blocking caused by crashed leaders, and derive Gatling's optimal number of parallel instances. We further study the impact of Gatling on predictable validity and present two variants that retain this property. Finally, our experiments confirm that Gatling can be used with off-the-shelf component protocols to achieve low latency without fine-tuning the component protocol for minimum latency.

==> commands.tex <==
\usepackage{chngcntr}
\usepackage{afterpage}
%
\usepackage{amsmath}
\makeatletter
\@ifclassloaded{acmart}{}{%
  \usepackage{amssymb}%
}
\makeatother
\usepackage{esvect}
\usepackage{footmisc}
\usepackage{float}
\usepackage[export]{adjustbox}
\usepackage{url}
\usepackage{commath}
\def\UrlBreaks{\do\/\do-}
%
\usepackage[nolist,nohyperlinks]{acronym}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{algorithm}
\usepackage{centernot}
\usepackage{wasysym}
\usepackage[inline]{enumitem}
\makeatletter
\@ifclassloaded{acmart}{}{%
  \usepackage{graphicx}%
}
\makeatother
\usepackage{multirow}
\usepackage{listings}
\usepackage{sidecap}
\makeatletter
\@ifclassloaded{acmart}{}{%
  \usepackage{hyperref}%
}
\makeatother
\usepackage[dvipsnames]{xcolor}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.97,0.97,0.97}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\small,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}

\lstset{style=mystyle}

\usepackage{longtable}
\usepackage{tikz}
\usepackage{algorithm}
\usepackage{wrapfig}
\usepackage{algpseudocode}
\usetikzlibrary{decorations.pathreplacing,positioning, arrows.meta, calc, patterns, fit, backgrounds, shapes, arrows, spy}
\tikzstyle{level 1}=[level distance=3cm, sibling distance=2cm]
\tikzstyle{level 2}=[level distance=3cm, sibling distance=2cm]
\tikzstyle{bag} = [text width=6em, text centered]
\tikzstyle{bagWide} = [text width=10em, text centered]
\usepackage{rotating}
\usepackage{pifont}
\usepackage{mathtools}
%
%
\makeatletter
\@ifclassloaded{lipics-v2021}{}{%
  \usepackage{subfig}%
}
\makeatother
\usepackage{dashrule}
\usepackage{xspace}
\usepackage{mdframed}
%
\usepackage{colortbl}
\usepackage{multirow}
\usepackage{pgfplots}
\usepackage{upgreek}
\pgfplotsset{compat = 1.3}
%
%
\usepackage{lscape}
\usepackage{cryptocode}
%
%
%
%
%
\newcommand{\vLineHeight}{3pt}
\newcommand{\hLineDistance}{2}
\newcommand{\numHLine}{7}
\newcommand{\mult}[2]{\pgfmathparse{#1*#2}\pgfmathresult}
\newcommand{\lengthofthing}{\mult{\hLineDistance}{\numHLine}}
%
%
%
%
%
%
%
%
\usepackage{enumitem}
\setlist[itemize]{parsep=0pt, topsep=0pt}
\setlist[enumerate]{parsep=0pt}
\setlist[description]{parsep=0pt, topsep=1pt}
%
%
\usepackage{soul}



%
%
%
%
%
%
%
%
%
%
%

%
\newcommand{\composite}{Gatling\xspace}

%
\newcommand{\nodes}{\ensuremath{\mathcal{N}}}

%
\newcommand{\ledger}{\ensuremath{\Lambda}}
\newcommand{\block}{\ensuremath{\mathsf{B}}}
\newcommand{\sparseledger}{\ensuremath{\hat{\mathcal{L}}}}
\newcommand{\chain}{\ensuremath{\mathcal{C}}}
\newcommand{\lstate}{\ensuremath{S}}
\newcommand{\tx}{\ensuremath{\mathsf{tx}}}
\newcommand{\capitaltx}{\ensuremath{\mathsf{Tx}}}
\newcommand{\rread}{\ensuremath{\mathsf{read}}}
\newcommand{\wwrite}{\ensuremath{\mathsf{write}}}
\newcommand{\execute}{\ensuremath{\mathsf{execute}}}
\newcommand{\genesis}{\ensuremath{\mathcal{G}}}
\newcommand{\deliveredLog}{\ensuremath{\mathsf{deliveredAnnotatedLog}}}

%
\newcommand{\daprot}{\ensuremath{\Pi^{DA}}}
\newcommand{\vidprot}{\ensuremath{\mathsf{VID}}}
\newcommand{\vabaprot}{\ensuremath{\Pi^{\mathsf{vaba}}}}
\newcommand{\disperseprot}{\ensuremath{\mathsf{Disperse}}}
\newcommand{\retrieveprot}{\ensuremath{\mathsf{Retrieve}}}
\newcommand{\verifyprot}{\ensuremath{\mathsf{Verify}}}
\newcommand{\vbaprot}{\ensuremath{\Pi^{\mathsf{VBA}}}}
\newcommand{\abprot}{\ensuremath{\Pi^{\mathsf{AB}}}}
\newcommand{\bcast}{\ensuremath{\mathsf{broadcast}}}
\newcommand{\deliver}{\ensuremath{\mathsf{deliver}}}

\newcommand{\view}{\ensuremath{\mathsf{v}}}
\newcommand{\PIcomponent}{\ensuremath{\Pi^{\mathrm{c}}}}
\newcommand{\PIcomposite}{\ensuremath{\Pi^{\mathrm{G}}}}

%
\newcommand{\deltaibt}{\ensuremath{T_{\mathrm{ipt}}}}
\newcommand{\deltaconf}{\ensuremath{T_{\mathrm{conf}}}}
\newcommand{\Tproposal}{\ensuremath{T^{\mathrm{prop}}}}
\newcommand{\Tvote}{\ensuremath{T^{\mathrm{vote}}}}
\newcommand{\proposalTime}{\ensuremath{T^{\mathrm{s}}}}

\def\Let#1#2{\State $#1\gets#2$}
\newcommand{\CommentLine}[1]{
    \State \(\triangleright\) \textit{#1}
}

\newcommand{\verifierAlg}[1]{{\color{blue} #1}}
\newcommand{\proverAlg}[1]{{\color{orange} #1}}
\def\Receive#1#2{\State $#1\dashleftarrow#2$}
\def\ReceiveIndented#1#2{\State \ \ \ \ \ $#1\dashleftarrow#2$}
\def\Send#1#2{\State $#1\dashrightarrow#2$}
\def\SendIndented#1#2{\State \ \ \ \ \ $#1\dashrightarrow#2$}
\def\Require#1{\State \textbf{require} #1}

\newcommand{\myparagraph}[1]{\smallskip\noindent\textbf{#1.} }

%
\newcommand{\newBlock}{\ensuremath{\mathsf{B}}}

\newcommand{\cbox}[1]{
	\begin{center}
		\underline{#1}
\end{center}}
\newcommand{\lbox}[1]{
	\begin{flushleft}
		\underline{#1}
\end{flushleft}}
\newcommand{\llbox}[1]{
	\begin{flushleft}
		#1
\end{flushleft}}
\newcommand{\rbox}[1]{
	\begin{flushright}
		\underline{#1}
\end{flushright}}

\mdfsetup{frametitlealignment=\center,innerleftmargin=5pt,innerrightmargin=3pt}
\newcommand{\mdframeSkip}{15pt}

\newenvironment{protocol}[1]{
	\begin{mdframed}[font=\small,frametitle={#1},frametitlerule=false,frametitlebackgroundcolor=white,splittopskip=\mdframeSkip,splitbottomskip=\mdframeSkip,startinnercode={\baselineskip=0cm}]}
	{\end{mdframed}}
\newenvironment{subprotocol}[1]{
	\begin{center}
		\rule{\textwidth}{1pt}\\
		\underline{\textbf{#1}}
	\end{center}
}	{}

%
\newtheorem{prop}{Proposition}
\newtheorem{conj}{Conjecture}
\makeatletter
\@ifclassloaded{lipics-v2021}{}{%
  \newtheorem{observation}{Observation}%
}
\makeatother
\newtheorem{myclaim}{Claim}
%


\usepackage{subcaption}
\usepackage{fontawesome5}
\usepackage{nicefrac}


\newcommand{\eps}{\ensuremath{\varepsilon}}

\newcommand{\negl}{\ensuremath{\operatorname{negl}}}
\newcommand{\poly}{\ensuremath{\operatorname{poly}}}
\newcommand{\Texec}{\ensuremath{T_{\mathrm{exec}}}}
\newcommand{\Tconf}{\ensuremath{T_{\mathrm{conf}}}}

\newcommand{\tS}{\ensuremath{\tau^{\mathrm{S}}}}
\newcommand{\tL}{\ensuremath{\tau^{\mathrm{L}}}}

\newcommand{\GST}{\ensuremath{\mathsf{GST}}}
%
\newcommand{\txs}{\ensuremath{\mathsf{txs}}}

%
%
\newcommand{\consistent}{\ensuremath{\asymp}}

\newcommand{\LOG}{\ensuremath{\uplambda}}

\newcommand{\qevict}[1]{\ensuremath{\mathcal{Q}_e(#1)}}

%
\newcommand{\AT}[3]{\ensuremath{\prescript{#1}{#2}{}#3}}

%
%

\newcommand{\TRUE}{\ensuremath{\mathtt{true}}}
\newcommand{\FALSE}{\ensuremath{\mathtt{false}}}
\newcommand{\UNDEFINED}{\ensuremath{\mathtt{undefined}}}

\newcommand{\CPa}{\ensuremath{\CP_{\mathrm{a}}}}
\newcommand{\CPh}{\ensuremath{\CP_{\mathrm{h}}}}

%
%

%
\makeatletter
\@ifclassloaded{IEEEtran}{%
  \newtheorem{theorem}{Theorem}
  \newtheorem{lemma}{Lemma}
  \newtheorem{definition}{Definition}
  \newtheorem{corollary}{Corollary}
  \newtheorem{remark}{Remark}
  \newtheorem{proposition}{Proposition}
}{%
  \@ifclassloaded{acmart}{%
    %
    %
    \let\definition\relax
    \let\enddefinition\relax
    \newtheorem{definition}{Definition}
    %
    %
    \AtEndPreamble{%
      \@ifundefined{remark}{%
        \theoremstyle{acmplain}%
        \newtheorem{remark}{Remark}[section]%
      }{}%
    }%
  }{%
    \@ifclassloaded{lipics-v2021}{}{%
      %
      \newtheorem{theorem}{Theorem}
      \newtheorem{lemma}{Lemma}
      \newtheorem{definition}{Definition}
      \newtheorem{corollary}{Corollary}
      \newtheorem{remark}{Remark}
      \newtheorem{proposition}{Proposition}
    }%
  }%
}%
\makeatother

\newcommand{\Prob}[1]{\ensuremath{\operatorname{Pr}\!\left[#1\right]}}
\newcommand{\Mean}[1]{\ensuremath{\operatorname{E}\!\left[#1\right]}}

\newcommand{\scriptspacing}[0]{\medmuskip=0mu\thickmuskip=0mu}

\newcommand{\myIconAdvCrash}{\faAngry[regular]\faDizzy[regular]}
\newcommand{\myIconAdvPartition}{\faAngry[regular]\faCommentSlash[regular]}
\newcommand{\myIconHonPartition}{\faCommentSlash[regular]}

\newcommand{\myTextHighlighted}[1]{\textcolor{myA16zAmber}{#1}}
\newcommand{\myTextHighlightedDescription}[0]{in \myTextHighlighted{orange}}
\newcommand{\myTextHighlightedTwo}[1]{\textcolor{jnSUDigitalGreen}{#1}}
\newcommand{\myTextHighlightedTwoDescription}[0]{in \myTextHighlightedTwo{green}}



==> lib/_boilerplate_base.tex <==
%
\PassOptionsToPackage{hyphens}{url}%
\makeatletter
\newcommand*{\@ifclassloadedlipicsoracmart}[2]{%
  \@ifclassloaded{acmart}{#2}{%
    \@ifclassloaded{lipics-v2021}{#2}{#1}%
  }%
}
\makeatother

\makeatletter
\@ifclassloadedlipicsoracmart{%
  \usepackage{hyperref}%
  \usepackage{graphicx}%
}{}
\makeatother


%
\usepackage{amsmath}
\makeatletter
\@ifclassloadedlipicsoracmart{%
  \let\proof\relax
  \let\endproof\relax
}{}
\makeatother
\makeatletter
\@ifclassloadedlipicsoracmart{%
  \usepackage{amsthm}%
}{}
\makeatother
\makeatletter
\@ifclassloadedlipicsoracmart{%
  \usepackage{amssymb}%
}{}
\makeatother
\usepackage{amsfonts}
\usepackage{mathtools}


%
\usepackage{shortsym}


%
%
\makeatletter
\@ifclassloaded{IEEEtran}{}{%
  \usepackage{IEEEtrantools}%
}
\makeatother
\allowdisplaybreaks


%
\let\labelindent\relax   %
%
\usepackage[shortlabels,inline]{enumitem}
\setlist[itemize]{leftmargin=1.25em}
\setlist[enumerate]{leftmargin=1.75em}
%
%


%
\usepackage[normalem]{ulem}


%
\usepackage{import}
\subimport{.}{_boilerplate_base_hyphenations.tex}
\subimport{.}{_boilerplate_base_mathenvironments.tex}
\subimport{.}{_boilerplate_base_math.tex}
\subimport{.}{_boilerplate_base_symbols.tex}
\subimport{.}{_boilerplate_base_textdecorations.tex}
\subimport{.}{_boilerplate_base_textabbreviations.tex}



==> lib/_boilerplate_base_hyphenations.tex <==
\hyphenation{a-vail-a-bil-i-ty}

\hyphenation{ac-count-a-bil-i-ty}
\hyphenation{ac-count-a-ble}
\hyphenation{ac-count-a-bly}

\hyphenation{led-ger}

\hyphenation{Na-ka-mo-to}

\hyphenation{white-pa-per}

\hyphenation{equi-vo-ca-tion}
\hyphenation{equi-vo-ca-ting}



==> lib/_boilerplate_base_math.tex <==
%

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\len}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}

%
%
%
\makeatletter
\let\oldabs\abs
\def\abs{\@ifstar{\oldabs}{\oldabs*}}
\let\oldlen\len
\def\len{\@ifstar{\oldlen}{\oldlen*}}
\let\oldnorm\norm
\def\norm{\@ifstar{\oldnorm}{\oldnorm*}}
\let\oldfloor\floor
\def\floor{\@ifstar{\oldfloor}{\oldfloor*}}
\let\oldceil\ceil
\def\ceil{\@ifstar{\oldceil}{\oldceil*}}
\makeatother


\newcommand{\cond}[0]{\ensuremath{\,\middle|\,}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


==> lib/_boilerplate_base_mathenvironments.tex <==
\theoremstyle{plain}
%
%
%
%
%
%
%
\newtheorem*{theorem*}{Theorem}
%
%
%
\newtheorem*{conjecture*}{Conjecture}
%

\theoremstyle{definition}
%
%
%
%
%



%
\makeatletter
\renewcommand*\env@matrix[1][*\c@MaxMatrixCols c]{%
    \hskip -\arraycolsep
    \let\@ifnextchar\new@ifnextchar
    \array{#1}}
\makeatother


==> lib/_boilerplate_base_symbols.tex <==
%

%
\usepackage{pifont}
%
%
\newcommand{\cmark}{\ding{52}}%
\newcommand{\xmark}{\ding{56}}%


%

\newcommand{\eqA}[0]{\ensuremath{\overset{\text{{(a)}}}{=}}}
\newcommand{\eqB}[0]{\ensuremath{\overset{\text{{(b)}}}{=}}}
\newcommand{\eqC}[0]{\ensuremath{\overset{\text{{(c)}}}{=}}}
\newcommand{\eqD}[0]{\ensuremath{\overset{\text{{(d)}}}{=}}}
\newcommand{\eqE}[0]{\ensuremath{\overset{\text{{(e)}}}{=}}}
\newcommand{\eqF}[0]{\ensuremath{\overset{\text{{(f)}}}{=}}}
\newcommand{\eqG}[0]{\ensuremath{\overset{\text{{(g)}}}{=}}}
\newcommand{\eqH}[0]{\ensuremath{\overset{\text{{(h)}}}{=}}}
\newcommand{\eqI}[0]{\ensuremath{\overset{\text{{(i)}}}{=}}}
\newcommand{\eqJ}[0]{\ensuremath{\overset{\text{{(j)}}}{=}}}
\newcommand{\eqK}[0]{\ensuremath{\overset{\text{{(k)}}}{=}}}
\newcommand{\eqL}[0]{\ensuremath{\overset{\text{{(l)}}}{=}}}

\newcommand{\neqA}[0]{\ensuremath{\overset{\text{{(a)}}}{\neq}}}
\newcommand{\neqB}[0]{\ensuremath{\overset{\text{{(b)}}}{\neq}}}
\newcommand{\neqC}[0]{\ensuremath{\overset{\text{{(c)}}}{\neq}}}
\newcommand{\neqD}[0]{\ensuremath{\overset{\text{{(d)}}}{\neq}}}
\newcommand{\neqE}[0]{\ensuremath{\overset{\text{{(e)}}}{\neq}}}
\newcommand{\neqF}[0]{\ensuremath{\overset{\text{{(f)}}}{\neq}}}
\newcommand{\neqG}[0]{\ensuremath{\overset{\text{{(g)}}}{\neq}}}
\newcommand{\neqH}[0]{\ensuremath{\overset{\text{{(h)}}}{\neq}}}
\newcommand{\neqI}[0]{\ensuremath{\overset{\text{{(i)}}}{\neq}}}
\newcommand{\neqJ}[0]{\ensuremath{\overset{\text{{(j)}}}{\neq}}}
\newcommand{\neqK}[0]{\ensuremath{\overset{\text{{(k)}}}{\neq}}}
\newcommand{\neqL}[0]{\ensuremath{\overset{\text{{(l)}}}{\neq}}}

\newcommand{\leqA}[0]{\ensuremath{\overset{\text{{(a)}}}{\leq}}}
\newcommand{\leqB}[0]{\ensuremath{\overset{\text{{(b)}}}{\leq}}}
\newcommand{\leqC}[0]{\ensuremath{\overset{\text{{(c)}}}{\leq}}}
\newcommand{\leqD}[0]{\ensuremath{\overset{\text{{(d)}}}{\leq}}}
\newcommand{\leqE}[0]{\ensuremath{\overset{\text{{(e)}}}{\leq}}}
\newcommand{\leqF}[0]{\ensuremath{\overset{\text{{(f)}}}{\leq}}}
\newcommand{\leqG}[0]{\ensuremath{\overset{\text{{(g)}}}{\leq}}}
\newcommand{\leqH}[0]{\ensuremath{\overset{\text{{(h)}}}{\leq}}}
\newcommand{\leqI}[0]{\ensuremath{\overset{\text{{(i)}}}{\leq}}}
\newcommand{\leqJ}[0]{\ensuremath{\overset{\text{{(j)}}}{\leq}}}
\newcommand{\leqK}[0]{\ensuremath{\overset{\text{{(k)}}}{\leq}}}
\newcommand{\leqL}[0]{\ensuremath{\overset{\text{{(l)}}}{\leq}}}

\newcommand{\ltA}[0]{\ensuremath{\overset{\text{{(a)}}}{<}}}
\newcommand{\ltB}[0]{\ensuremath{\overset{\text{{(b)}}}{<}}}
\newcommand{\ltC}[0]{\ensuremath{\overset{\text{{(c)}}}{<}}}
\newcommand{\ltD}[0]{\ensuremath{\overset{\text{{(d)}}}{<}}}
\newcommand{\ltE}[0]{\ensuremath{\overset{\text{{(e)}}}{<}}}
\newcommand{\ltF}[0]{\ensuremath{\overset{\text{{(f)}}}{<}}}
\newcommand{\ltG}[0]{\ensuremath{\overset{\text{{(g)}}}{<}}}
\newcommand{\ltH}[0]{\ensuremath{\overset{\text{{(h)}}}{<}}}
\newcommand{\ltI}[0]{\ensuremath{\overset{\text{{(i)}}}{<}}}
\newcommand{\ltJ}[0]{\ensuremath{\overset{\text{{(j)}}}{<}}}
\newcommand{\ltK}[0]{\ensuremath{\overset{\text{{(k)}}}{<}}}
\newcommand{\ltL}[0]{\ensuremath{\overset{\text{{(l)}}}{<}}}

\newcommand{\llA}[0]{\ensuremath{\overset{\text{{(a)}}}{\ll}}}
\newcommand{\llB}[0]{\ensuremath{\overset{\text{{(b)}}}{\ll}}}
\newcommand{\llC}[0]{\ensuremath{\overset{\text{{(c)}}}{\ll}}}
\newcommand{\llD}[0]{\ensuremath{\overset{\text{{(d)}}}{\ll}}}
\newcommand{\llE}[0]{\ensuremath{\overset{\text{{(e)}}}{\ll}}}
\newcommand{\llF}[0]{\ensuremath{\overset{\text{{(f)}}}{\ll}}}
\newcommand{\llG}[0]{\ensuremath{\overset{\text{{(g)}}}{\ll}}}
\newcommand{\llH}[0]{\ensuremath{\overset{\text{{(h)}}}{\ll}}}
\newcommand{\llI}[0]{\ensuremath{\overset{\text{{(i)}}}{\ll}}}
\newcommand{\llJ}[0]{\ensuremath{\overset{\text{{(j)}}}{\ll}}}
\newcommand{\llK}[0]{\ensuremath{\overset{\text{{(k)}}}{\ll}}}
\newcommand{\llL}[0]{\ensuremath{\overset{\text{{(l)}}}{\ll}}}

\newcommand{\geqA}[0]{\ensuremath{\overset{\text{{(a)}}}{\geq}}}
\newcommand{\geqB}[0]{\ensuremath{\overset{\text{{(b)}}}{\geq}}}
\newcommand{\geqC}[0]{\ensuremath{\overset{\text{{(c)}}}{\geq}}}
\newcommand{\geqD}[0]{\ensuremath{\overset{\text{{(d)}}}{\geq}}}
\newcommand{\geqE}[0]{\ensuremath{\overset{\text{{(e)}}}{\geq}}}
\newcommand{\geqF}[0]{\ensuremath{\overset{\text{{(f)}}}{\geq}}}
\newcommand{\geqG}[0]{\ensuremath{\overset{\text{{(g)}}}{\geq}}}
\newcommand{\geqH}[0]{\ensuremath{\overset{\text{{(h)}}}{\geq}}}
\newcommand{\geqI}[0]{\ensuremath{\overset{\text{{(i)}}}{\geq}}}
\newcommand{\geqJ}[0]{\ensuremath{\overset{\text{{(j)}}}{\geq}}}
\newcommand{\geqK}[0]{\ensuremath{\overset{\text{{(k)}}}{\geq}}}
\newcommand{\geqL}[0]{\ensuremath{\overset{\text{{(l)}}}{\geq}}}

\newcommand{\gtA}[0]{\ensuremath{\overset{\text{{(a)}}}{>}}}
\newcommand{\gtB}[0]{\ensuremath{\overset{\text{{(b)}}}{>}}}
\newcommand{\gtC}[0]{\ensuremath{\overset{\text{{(c)}}}{>}}}
\newcommand{\gtD}[0]{\ensuremath{\overset{\text{{(d)}}}{>}}}
\newcommand{\gtE}[0]{\ensuremath{\overset{\text{{(e)}}}{>}}}
\newcommand{\gtF}[0]{\ensuremath{\overset{\text{{(f)}}}{>}}}
\newcommand{\gtG}[0]{\ensuremath{\overset{\text{{(g)}}}{>}}}
\newcommand{\gtH}[0]{\ensuremath{\overset{\text{{(h)}}}{>}}}
\newcommand{\gtI}[0]{\ensuremath{\overset{\text{{(i)}}}{>}}}
\newcommand{\gtJ}[0]{\ensuremath{\overset{\text{{(j)}}}{>}}}
\newcommand{\gtK}[0]{\ensuremath{\overset{\text{{(k)}}}{>}}}
\newcommand{\gtL}[0]{\ensuremath{\overset{\text{{(l)}}}{>}}}

\newcommand{\ggA}[0]{\ensuremath{\overset{\text{{(a)}}}{\gg}}}
\newcommand{\ggB}[0]{\ensuremath{\overset{\text{{(b)}}}{\gg}}}
\newcommand{\ggC}[0]{\ensuremath{\overset{\text{{(c)}}}{\gg}}}
\newcommand{\ggD}[0]{\ensuremath{\overset{\text{{(d)}}}{\gg}}}
\newcommand{\ggE}[0]{\ensuremath{\overset{\text{{(e)}}}{\gg}}}
\newcommand{\ggF}[0]{\ensuremath{\overset{\text{{(f)}}}{\gg}}}
\newcommand{\ggG}[0]{\ensuremath{\overset{\text{{(g)}}}{\gg}}}
\newcommand{\ggH}[0]{\ensuremath{\overset{\text{{(h)}}}{\gg}}}
\newcommand{\ggI}[0]{\ensuremath{\overset{\text{{(i)}}}{\gg}}}
\newcommand{\ggJ}[0]{\ensuremath{\overset{\text{{(j)}}}{\gg}}}
\newcommand{\ggK}[0]{\ensuremath{\overset{\text{{(k)}}}{\gg}}}
\newcommand{\ggL}[0]{\ensuremath{\overset{\text{{(l)}}}{\gg}}}


%

\usepackage{dsfont}
\newcommand{\Ione}{{\mathds{1}}}


%

\DeclareRobustCommand{\svdots}{%
    \vcenter{%
        \offinterlineskip%
        \hbox{.}%
        \vskip0.25\normalbaselineskip%
        \hbox{.}%
        \vskip0.25\normalbaselineskip%
        \hbox{.}%
    }%
}
\DeclareRobustCommand{\sddots}{%
    \vcenter{%
        \offinterlineskip%
        %
        \hbox{.\hspace{0.5\normalbaselineskip}}%
        \vskip0.25\normalbaselineskip%
        %
        \hbox{\hspace{0.25\normalbaselineskip}.\hspace{0.25\normalbaselineskip}}%
        \vskip0.25\normalbaselineskip%
        %
        \hbox{\hspace{0.5\normalbaselineskip}.}%
    }%
}
\DeclareRobustCommand{\scdots}{%
    \vcenter{%
        \offinterlineskip%
        \hbox{.\,.\,.}%
    }%
}

%
%
%



==> lib/_boilerplate_base_textabbreviations.tex <==
\usepackage{xspace}

\newcommand{\cf}[0]{cf.\xspace}
\newcommand{\ie}[0]{\emph{i.e.}\xspace}
\newcommand{\eg}[0]{\emph{e.g.}\xspace}
\newcommand{\vs}[0]{vs.\xspace}
\newcommand{\aka}[0]{a.k.a.\xspace}




==> lib/_boilerplate_base_textdecorations.tex <==
%

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
                \node[shape=circle,draw=black,text=black,inner sep=2pt] (char) {\footnotesize #1};}}

\newcommand*\circledScript[1]{\tikz[baseline=(char.base)]{
                \node[shape=circle,draw=black,text=black,inner sep=2pt] (char) {\scriptsize #1};}}
\newcommand*\circledScriptGray[1]{\tikz[baseline=(char.base)]{
                \node[shape=circle,draw=black,text=black,inner sep=2pt,fill=black!10] (char) {\scriptsize #1};}}
\newcommand*\circledScriptGraySlim[1]{\tikz[baseline=(char.base)]{
                \node[shape=circle,draw=black,text=black,inner sep=1pt,fill=black!10] (char) {\scriptsize #1};}}

\newcommand*\circledScriptBlackSlim[1]{\tikz[baseline=(char.base)]{
                \node[shape=circle,draw=none,fill=black,text=white,inner sep=1pt] (char) {\scriptsize #1};}}

\newcommand*\circledTiny[1]{\tikz[baseline=(char.base)]{
                \node[shape=circle,draw=black,text=black,inner sep=2pt] (char) {\tiny #1};}}
\newcommand*\circledTinyGray[1]{\tikz[baseline=(char.base)]{
                \node[shape=circle,draw=black,text=black,inner sep=2pt,fill=black!10] (char) {\tiny #1};}}
\newcommand*\circledTinyGraySlim[1]{\tikz[baseline=(char.base)]{
                \node[shape=circle,draw=black,text=black,inner sep=1pt,fill=black!10] (char) {\tiny #1};}}

\newcommand*\circledTinyBlackSlim[1]{\tikz[baseline=(char.base)]{
                \node[shape=circle,draw=none,fill=black,text=white,inner sep=1pt] (char) {\tiny #1};}}



==> lib/defer.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\RequirePackage{expl3}
\RequirePackage{scontents}


%
%
%
\ExplSyntaxOn

%
%
%
\cs_new_protected:Npn \defer_new_group:nn #1 #2 {
  %
  \bool_if_exist:cF { l__defer_#1 _bool } { \bool_new:c { l__defer_#1 _bool } }
  %
  \tl_set:Nx \l_tmpa_tl { \tl_lower_case:n {#2} }
  %
  \str_if_eq:VnTF \l_tmpa_tl {deferred}
    { \bool_set_true:c  { l__defer_#1 _bool } }
    { \bool_set_false:c { l__defer_#1 _bool } }
}


%
%
%

%
%
\NewDocumentCommand{\newdefergroup}{m O{deferred}}{
  \defer_new_group:nn {#1}{#2}
}

%
%
\NewDocumentEnvironment{ifdeferred}{m +b}{%
  \bool_if:cT { l__defer_#1 _bool } { #2 }%
}{}

%
%
\NewDocumentEnvironment{ifnotdeferred}{m +b}{%
  \bool_if:cF { l__defer_#1 _bool } { #2 }%
}{}

%
%
%
\NewDocumentEnvironment{defer}{m +b}{%
  \bool_if:cTF { l__defer_#1 _bool }{%
    %
    \Scontents[store-cmd=defer@#1,print-cmd=false]{#2}%
  }{%
    %
    #2%
  }%
}{}

%
%
\NewDocumentCommand{\printdefergroup}{m}{%
  %
  \foreachsc{defer@#1}%
}

\ExplSyntaxOff

%
%
%

%
%
%
%
\NewDocumentCommand{\deferredproof}{m m}{%
  \begin{ifdeferred}{#1}%
    Proof of \cref{#2} is deferred to \cref{sec:deferred-#1}.%
  \end{ifdeferred}%
}

%
%
%
\NewDocumentCommand{\deferredsection}{m m}{%
  \begin{ifdeferred}{#1}%
    \section{#2}%
    \label{sec:deferred-#1}%
    \printdefergroup{#1}%
  \end{ifdeferred}%
}


==> lib/utils.tex <==
\IfFileExists{version-string.txt}{%
  \newread\versionfile
  \openin\versionfile=version-string.txt
  \read\versionfile to \myVersionString
  \closein\versionfile
}{}
